Step out of KG: Knowledge Graph Completion via Knowledgeable Retrieval and Reading Comprehension

Knowledge graphs, as the cornerstone of many AI applications, usually face serious incompleteness problems. In recent years, there have been many efforts to study automatic knowledge graph completion (KGC), most of which use existing knowledge to infer new knowledge. However, in our experiments, we find that not all relations can be obtained by inference, which constrains the performance of existing models. To alleviate this problem, we propose a new model based on information retrieval and reading comprehension, namely IR4KGC. Specifically, we pre-train a knowledge-based information retrieval module that can retrieve documents related to the triples to be completed. Then, the retrieved documents are handed over to the reading comprehension module to generate the predicted answers. In experiments, we find that our model can well solve relations that cannot be inferred from existing knowledge, and achieve good results on KGC datasets.

==> tables/4.relations.tex <==
\begin{table*}[hbt!]
  \centering
  \hspace*{-0.32cm}
  \setlength\tabcolsep{5.5pt}
  \scalebox{0.8}{
  \begin{tabular}{lcc}
  \toprule
    Dataset & Inferable Relations &  Uninferable Relations \\ 
  \midrule
  \multirow{7}{*}{CoDEx-M} & \textit{country} (P17) & \textit{cause of death} (P509)  \\
  & \textit{languages spoken, written or signed} (P1412) & \textit{place of burial} (P119)   \\
  & \textit{occupation} (P106) & \textit{place of birth} (P19)  \\
  & \textit{country of citizenship} (P27) & \textit{place of death} (P20)  \\
  & \textit{member of} (P463) & \textit{religion or worldview} (P140)  \\
  & \textit{located in the administrative territorial entity} (P131) & \textit{child} (P40)  \\
  & \textit{headquarters location} (P159) & \textit{director} (P57)  \\
  \midrule
  \multirow{7}{*}{FB15K-237-N}   & \textit{/influence/influence\_node/influenced\_by} & \textit{/people/cause\_of\_death/people}  \\ 
  & \textit{/location/location/time\_zones} & \textit{/people/person/place\_of\_birth}  \\
  & \textit{/people/person/nationality} & \textit{/film/film/featured\_film\_locations}  \\
  & \textit{/location/country/official\_language} & \textit{/people/deceased\_person/place\_of\_death}  \\
  & \textit{/people/ethnicity/languages\_spoken} & \textit{/music/artist/origin}  \\
  & \textit{/sports/sports\_team/sport} & \textit{/education/educational\_institution/colors}  \\
  & \textit{/tv/tv\_program/genre} & \textit{/organization/organization\_founder/organizations\_founded}  \\
  \bottomrule
  \end{tabular}
  }
  \vspace{-0.1cm}
  \caption{Inferable relations and uninferable relations that we annotate on the KGC datasets.}
  \label{tab:relation_annotation}
  \vspace{-0.2cm}
\end{table*}

==> tables/5.case.tex <==
 \begin{table*}[t]
  \centering
  \hspace*{-0.32cm}
\setlength\tabcolsep{5.5pt}
  \scalebox{0.9}{
  \begin{tabular}{ccp{10cm}}
    \toprule
    Triple Query & Model &  \makebox[10cm][c]{Retrieved Document}  \\ 
  \midrule
  \multirow{17}{*}{(Lebron James, \textit{place of birth}, ?)} & \multirow{2}{*}{BM25+MRC}  &  This page lists career accomplishments of the American professional basketball player LeBron James. \\
  \cmidrule(lr){2-3}
  & \multirow{8}{*}{RAG} & Fiasco was born Wasalu Muhammad Jaco on February 16, 1982 in Chicago, Illinois. Fiasco is of West African descent, one of nine children of Shirley, a gourmet chef, and Gregory, an engineer. His father, a member of the Black Panther Party, was a prolific African drummer, karate teacher, operating plant engineer, and owner of karate schools and army surplus stores. Fiasco was raised Muslim on the West Side of Chicago on Madison Terrace housing project. At the age of three, Fiasco began taking martial arts classes.   \\
  \cmidrule(lr){2-3}
  & \multirow{7}{*}{IR4KGC} &  James was selected to the All-NBA First Team twelve times (all-time record), made the All-Defensive First Team five times, and has played in sixteen All-Star Games, in which he was selected All-Star MVP three times. \textbf{James played basketball for St. Vincent–St. Mary High School in his hometown of Akron, Ohio}, where he was heavily touted by the national media as a future NBA superstar. A prep-to-pro, he joined Cleveland in 2003 as the first draft pick.  \\
  \midrule
  \multirow{27}{*}{(Avatar, \textit{director}, ?)} & \multirow{8}{*}{BM25+MRC}  &  On April 27, 2017, the release dates for all four sequels were ultimately announced: December 18, 2020 for Avatar 2, December 17, 2021 for Avatar 3, December 20, 2024 for Avatar 4, and December 19, 2025 for Avatar 5. The films will be released in Dolby Vision. \textbf{New crew members include cinematographer Russell Carpenter, who worked with Cameron on True Lies and Titanic}, and Aashrita Kamath, who will act as art director on all four sequels. \\
  \cmidrule(lr){2-3}
  & \multirow{10}{*}{RAG} & UiPath was founded in 2005 by the Romanian entrepreneurs, Daniel Dines and Marius Tirca, is a global software company that develops a platform for Robotic Process Automation (RPA or RPAAI). The company started from Bucharest, Romania and later opened offices in London, New York, Bengaluru, Singapore, and Tokyo. In 2017, the company reported 590 employees and moved its headquarters to New York to be closer to its international customer base, which rose to 700 customers from 100 in 2016. In August 2015, UiPath closed an initial seed funding round of \$1.6 million led by the Earlybird Venture Capital.   \\
  \cmidrule(lr){2-3}
  & \multirow{9}{*}{IR4KGC} &  \textbf{Avatar (marketed as James Cameron's Avatar)} is a 2009 American epic science fiction \textbf{film directed, written, produced, and co-edited by James Cameron} and stars Sam Worthington, Zoe Saldana, Stephen Lang, Michelle Rodriguez, and Sigourney Weaver. The film is set in the mid-22nd century when humans are colonizing Pandora, a lush habitable moon of a gas giant in the Alpha Centauri star system, in order to mine the mineral unobtanium, a room-temperature superconductor.This property of Unobtanium is stated in movie guides, rather than in the film.  \\
  \bottomrule
  \end{tabular}
  }
  \vspace{-0.1cm}
  \caption{For different triple queries, we give the most relevant document retrieved by different models. For display purposes, we have \textbf{bolded} the parts of the document that contain the answer to the corresponding triple query.}
  \label{tab:case_study}
  \vspace{-0.2cm}
  \end{table*}
